Towards Sample-efficient Overparameterized Meta-learning

An overarching goal in machine learning is to build a generalizable model with few samples. To this end, overparameterization has been the subject of immense interest to explain the generalization ability of deep nets even when the size of the dataset is smaller than that of the model. While the prior literature focuses on the classical supervised setting, this paper aims to demystify overparameterization for meta-learning. Here we have a sequence of linear-regression tasks and we ask: (1) Given earlier tasks, what is the optimal linear representation of features for a new downstream task? and (2) How many samples do we need to build this representation? This work shows that surprisingly, overparameterization arises as a natural answer to these fundamental meta-learning questions. Specifically, for (1), we first show that learning the optimal representation coincides with the problem of designing a task-aware regularization to promote inductive bias. We leverage this inductive bias to explain how the downstream task actually benefits from overparameterization, in contrast to prior works on few-shot learning. For (2), we develop a theory to explain how feature covariance can implicitly help reduce the sample complexity well below the degrees of freedom and lead to small estimation error. We then integrate these findings to obtain an overall performance guarantee for our meta-learning algorithm. Numerical experiments on real and synthetic data verify our insights on overparameterized meta-learning.

==> sections/bc/intro_05_23.tex <==
\section{Introduction}\label{sec:intro}



%Meta-learning (and multi-task learning) has proved to be a powerful technique when available training data is limited. The central idea is exploiting the information (e.g.~training data) provided by earlier related tasks to quickly adapt a new task using few samples. This idea has a rich history \cite{caruana1997multitask,baxter2000model} and has shown promise in modern machine learning tasks, e.g., in image classification \cite{deng2009imagenet}, machine translation \cite{bojar2014findings} and reinforcement learning \cite{finn2017model}, all of which may involve numerous tasks to be learned with limited data per task.

In a multitude of machine learning (ML) tasks with limited data, it is crucial to build accurate models in a sample-efficient way. This goal proves to be especially challenging when the features are high-dimensional, as is often the case in modern ML problems. Constructing a simple yet informative representation of features is a critical component of learning a model that generalizes well to an unseen test set. Representation learning, which dates back to \cite{caruana1997multitask,baxter2000model}, aims to jointly utilize information from the training data of multiple related tasks. Such information transfer is the backbone of modern transfer and multitask learning and finds ubiquitous applications in image classification \citep{deng2009imagenet}, machine translation \citep{bojar2014findings} and reinforcement learning \citep{finn2017model}, all of which may involve numerous tasks to be learned\footnote{In our setting, each task is parameterized by a vector in $\R^d$ and we learn this task vector given task data (features and labels). See Phase 1 in Section 2 for details.} with limited data per task. 
%for exact definition of task and feature.} 
%\mf{we can also comment on ideas behind `dictionary learning' related to rep learning? (not too urgent)---given the short time we can ignore this one}


In this paper, we focus on the fundamental problem of meta-learning with linear features. \so{While deep nets are nonlinear, recent advances showed that linearized problems such as kernel regression (e.g., via neural tangent kernel \cite{}) provides a good proxy to understand the theoretical properties of practical deep nets which are often highly overparameterized. Such theoretical understanding --such as inductive bias of gradient descent or double descent phenomena \cite{}-- has so far been limited to classical supervised setting where we have a single task under consideration. At a high-level, a core goal in this paper is building onto these works to develop a theoretical understanding of overparameterized meta-learning.}

\input{icml2021/sections/notation_table}

\an{The notation introduced here is either reintroduced later or does not appear again. @Samet @Yue do you think it might be better to replace with just text?}

Our meta-learning strategy consists of two phases \so{similar in spirit to \cite{tripuraneni2020provable,kong2020meta}}. In the representation learning phase, we learn a linear representation from a collection of $\ntask$ earlier tasks, with $\nspt$ training samples per task. %$\Sc=(\x_{ij},y_{ij})_{(i,j)=(1,1)}^{(\ntask,\nspt)}$ 
%\mf{should we move the regression setup here, from sec 2? Can explain the notation: for each regression problem, $x$ is the features, $\beta$ the task vector, there's additive noise. We can say this is the simplest setup that we use in our theoretical analysis, while we also experimentally explore the more general nonlinear setting... Or, if we decide to keep things high-level here, the regression setup should appear at the start of sec 2, and we refer to that here in the intro.} 
Let $(\x_{ij},y_{ij})$ be the $j$th training sample from task $i$ and we collect training samples from all tasks in the set $\Sc=\{(\x_{ij},y_{ij})\}\subset\R^d\times \R$. Denote $\ntot=\ntask\times \nspt = |\Sc|$. The goal of this stage is to output a \emph{representation matrix}
%linear representation
\begin{align}%:\x\rightarrow\Ar(\Sc)
\hbLa:=\hbLa(\Sc)\in\R^{\Rr\times d},\label{meta train eq}
\end{align}
that can be used to map raw input features to a linear feature map of dimension $R$. 
%where $\Rr$ is the embedding dimension \mf{unclear what embedding dimension means here. We can just say a representation of dimension $R$.}
%\mf{not sure if the $\Ar(\Sc)$ notation above helps. We can remove; just say given data, we find a matrix $\Lambda$.}---\mf{actually OK to jkeep it, makes it clear it depends on both features and labels}


In the second phase (few-shot learning), we are given a new task with data $\FS=\{(\x_{i},y_{i})\}_{i=1}^{\nfs}$, with possibly very small $\nfs$.  We use the representation $\hbLa$ to transform the input features to obtain a generalizable model $\bala$ by minimizing the empirical risk
\begin{align}
\Lch_{\FS}(\bal)=\frac{1}{\nfs}\sum_{i=1}^{\nfs}\ell(y_i,\bal^T\hbLa\x_i).\label{few shot eq}
\end{align}

\input{icml2021/sections/figure1}
Existing analysis of algorithms for both the meta-training and few-shot phases have typically focuses on the classical \emph{underparameterized regime}: when the sample size is larger than the degrees of freedom (DoF) of the problem. This leads to sample size requirements of $\Omega(\Rr d)$ for \eqref{meta train eq} and $\Omega(\Rr)$ for \eqref{few shot eq}. These works are also often focused on learning simplistic representations, where $\hbLa$ is simply a subspace (i.e.~orthonormal rows). However, the recent literature in deep learning makes it clear that the overparameterized regime is of significant interest for both problems. Deep networks are stellar representation learners despite containing many more parameters than the sample size. Additionally, the few-shot learning literature demonstrates that very few samples --often much fewer than the representation dimension-- can be sufficient for successful adaptation to an unseen task. For example, \cite{finn2017model} (MAML) and \cite{vinyals2016matching} successfully use a transfer learning method that adapts a pre-trained model, with $112980$ parameters, to downstream tasks with only 1-5 new training samples. 

In Figure~\ref{fig:fs_double_descent} a.,
a pretrained ResNet50 network on Imagenet (representation learning phase) was utilized to obtain a feature-representation for classification on CIFAR-10. After reducing the dimensionality to $r$ via PCA, the resultant features are to train a logistic regression classifier on CIFAR-10 with $k$ examples from each class (few-shot phase). The figure depicts the test error obtained using projected test features as a function of $r$. The interpolation threshold (i.e., when accurate fit for data happens) is indicated by the dashed line, and can be seen to coincide exactly with the location of the double-descent peak ($k=r$).
The benefits of overparameterization and double-descent in the few-shot phase are observed in a transfer learning task for image classification; for all choices of $k$ the accuracies are observed to be markedly higher in the overparameterized regime. 

\ys{The double descent behavior and the benefit of overparameterization is theoretically investigated in recent works \cite{mei2019generalization, wu2020optimal}. In Figure~\ref{fig:fs_double_descent} b., we apply our proposed meta-learning algorithm with arbitrary dimensional representation, and plot the error for learning the downstream task. Our proposed optimal shaping shows its optimality in overparameterized regime.}

The previous discussion motivates the following fundamental questions.
\begin{quote}
\textbf{Q1:} What is the optimal representation $\hbLa \in \R^{\Rr\times d}$ for minimal few-shot risk?\\
\textbf{Q2:} How to meta-learn in the overparameterized regime $\ntot\ll \Rr d$ and $\nfs\ll \Rr$?
\end{quote}
%propose meta-learning procedures that involve dimension reduction, clustering and few-shot learning. Here a low-dimensional task subspace is used as the search space for few-shot learning for the new task. Another related approach
%\cite{du2020few,tripuraneni2020provable}
%sets up a nonconvex optimization problem with matrix factors of appropriate sizes, which captures the low dimensional structure. One can apply gradient descent to this nonconvex problem, and studying its behavior requires a nontrivial landscape analysis of the matrix factorization problem.  

\noindent\textbf{Contributions:} Towards answering these, we make several key contributions to the finite-sample understanding of \emph{linear} meta-learning, under assumptions discussed in Section \ref{sec:setup}.  As described below, our results are enabled by studying a general data/task model with \emph{arbitrary task covariance $\bSt$ and feature covariance $\bSi$} which allows for a rich set of observations.
%\mf{say clearly the theoretical contributions are for the specific setup described in sec 2.}
%This is as opposed to comparable works which assume low-rank task or identity-like features}.

%representationexplaining how representation learning and few-shot learning can be accomplished with much fewer training samples than the model size.% in the overparameterized regime with 

%Our numerical experiments reveal that, in practice, representation learning happens in the over-parameterized regime.  We also demonstrate that, during few-shot learning, representation dimension can in fact be larger than the available few-shot sample size and unlike conventional wisdom, small representations can hurt. Both of these highlight a need for a meta-learning theory where sample size is smaller than the DoF.

%\rd{\noindent$\bullet$ \textbf{Empirical insights:} Our numerical experiments as well as prior literature demonstrate that, in practice, deep nets learn stellar representations despite being highly over-parameterized. We also demonstrate that, for $k$-shot learning, representation dimension is typically larger than the few-shot sample size which is as small as $2$ for 1-shot binary classification! In fact, representations with dimension smaller than $k$ can demonstrably hurt the performance (see Fig.~ \ref{fig:fs_double_descent} and \ref{fig3}). These highlight the need for a deeper theoretical understanding of over-parameterized meta-learning.}
%\mf{commented out `empirical insights' which was repetitive and not adding much}
%\ys{I believe it's important to link to empirical nn stuff as that's the motivation}
%\mf{right, but the parag text that was here wasn't good enough.}
%\mf{actually let's expand the empirical motivation in the parag before contributions, make a good argument there. then no need to have it here.}

$\bullet$ \textbf{Populational: Optimal representation.} We first study \textbf{Q1} in the population sense, which means we obtain the optimal representation matrix $\bLa$ with known distribution of tasks and features. %We answer this question by establishing an equivalence between the optimal linear representation and generalized ridge regression over the raw features (see Sec~\ref{sec:opt_rep}). 
Algorithm \ref{algo:opt rep} is the primary algorithm. Unlike simplistic subspace projections, the right representation for optimized few-shot performance can in fact be a high-dimensional map with $R\gg \nfs$ addressing \textbf{Q1} and \textbf{Q2}. In contrast to subspace-based schemes which discard certain features, $\hbopt$ shapes the feature covariance to emphasize informative features over less informative ones. We show that, the minimum excess risk of few-shot learning, instead of both feature covariance $\bSi$ and task covariance $\B$, depends on a ``summary'' variable (we call it canonical covariance) $\Bbar = \sbSi\B\sbSi$, used for dictating design of meta-learning algorithm.
%, and the optimal representation depends on $\Bbar$ after whitening the features. The goal of representation learning is to estimate $\Bbar$ in the empirical sense (where we need to estimate the distributions from data).

$\bullet$ \textbf{Empirical: Representation learning.} We study representation learning for linear regression tasks using established moment-based estimator (precisely defined in Section \ref{sec:meta train}), and specialize the bound for arbitrary $\Bbar$. We answer \textbf{Q2} in that, when $\bSi$ and $\Bbar$ have spiked eigenvalues and are aligned, we define the \emph{effective rank}s of $\bSi$ and $\Bbar$ and the proposed estimator succeeds with $\ntot = \order{\mathrm{rank}_{\mathrm{eff}}(\bSi)(\mathrm{rank}_{\mathrm{eff}}(\Bbar))^2}$. We check the spike of eigenvalue for MNIST dataset. The features are images and the data are the vector for linear SVM classifier. (Define...) The canonical alignment is $0.32$ and the task alignment is $0.18$.

$\bullet$ \textbf{Empirical: Few-shot learning:} In practice, $\hbopt$ is unattainable due to finite sample ($\ntot<\infty$) during the representation learning phase. We establish robustness guarantees under finite $\ntot$ to provide an end-to-end guarantee for two phases in terms of $\hbopt$. This also uncovers a sweet spot between subspace-based approaches and optimal-shaping schemes: As $\ntot$ decreases, it becomes more preferable to use a smaller $\Rr$ due to inaccurate estimate of to $\hbopt$. This explains why, in practice, lower dimensional representations may be preferable (see Fig. \ref{fig2} for details).


\iffalse

\noindent$\bullet$ \textbf{Representation learning.} 
%We study representation learning quality for \clr{established} moment-based algorithms 
We study representation learning for linear regression tasks using established moment-based algorithms (precisely defined in Section \ref{sec:meta train}), 
and formalize \emph{how feature-task interaction governs learning}. Specializing our bounds to the case of a rank-$\rt$ task covariance $\bSt$ and a ``spiked" (approximately low-rank) feature covariance $\bSi$ reveals that sample complexity for learning the task subspace is governed by the \emph{spectral alignment of the task \& feature covariances} and can go well below the DoF $\order{\rt d}$, answering \textbf{Q2}. Surprisingly, if this alignment is sufficiently strong, simple PCA estimator on the empirical feature covariance can be preferable to more sophisticated methods (see Fig. \ref{fig2}(a)). We motivate the task-feature alignment by the clustered features in Figure \ref{fig:fs_double_descent} b. Suppose we have a few binary classification tasks for representation learning, where each class contains features in a cluster. The tasks are the normal vectors of the decision boundaries. The column/row space task covariance, as well as the principal components of $\bSi$, is the span of cluster centers. They are low dimensional if cluster centers span a low dimensional subspace. 

\iffalse
\setlength{\textfloatsep}{.5em}
\begin{figure}[htbp!]
\centering
\vspace{-1em}
\includegraphics[width =0.9\linewidth]{icml2021/figs/GMM3.png}
\vspace{-2.5em}
\caption{Clustered data for representation learning. Each task corresponds to a binary classification problem between two arbitrary clusters, where the decision boundary is a hyperplane. $\mathrm{col}(\B) = \mathrm{span}(\mathrm{centers})$, and the principal subspace of $\bSi$ is $\mathrm{span}(\mathrm{centers})$.\\
\textcolor{blue}{TODO: Find the tasks on the feature maps obtained by Imagenet and verify feature-task alignment.}} 
\label{fig:cluster}
\end{figure} 
\fi


When specialized to the case with uninformative features ($\bSi=\Iden$), we show that $\order{\rt d}$ samples are sufficient when $\nspt\gtrsim \order{\rt}$ \emph{achieving optimal sample size} and improving over prior bounds of $\order{\rt^2 d}$ \cite{tripuraneni2020provable}. Importantly, this leads to the critical finding that, for fixed total sample size $\ntot$, \emph{both $\nspt$ and $\ntask$ should be reasonably large} for this near-optimal performance (see Fig.~\ref{fig2}(b) for details). 

%to learn the taskthe sample complexity analysis showing that the span of tasks can be learned from $DoF = \order{d\rt}$ samples, compared to $\order{d\rt^2}$ in \cite{tripuraneni2020provable}, which is proven in \cite{tripuraneni2020provable} as information theoretically optimal \mf{explain better}. We further show how the sample complexity can be drastically reduced from $DoF=\order{d\rt}$ to $\order{\rt}$ as a function of alignment and the choice of MoM algorithm.

%connecting optimal linear representation to a generalized ridge regression over the raw features.%optimally-shaped




\noindent$\bullet$ \textbf{Few-shot learning:} With access to infinite representation learning samples, what is the \emph{optimal representation} $\hbopt$? For least-squares regression, we answer this question by establishing an equivalence between the optimal linear representation and generalized ridge regression over the raw features (see Sec~\ref{sec:few shot}). This reveals that unlike simplistic subspace projections, the right representation for optimized few-shot performance can in fact be a high-dimensional map with $\Rr\gg \nfs$ addressing \textbf{Q1} and \textbf{Q2}. In contrast to subspace-based schemes which discard certain features, $\hbopt$ shapes the feature covariance to emphasize informative features over less informative ones. In practice, $\hbopt$ is unattainable due to finite sample ($\ntot<\infty$) during the representation learning phase. We establish robustness guarantees under finite $\ntot$ to provide an end-to-end guarantee for two phases in terms of $\hbopt$. This also uncovers a sweet spot between subspace-based approaches and optimal-shaping schemes: As $\ntot$ decreases, it becomes more preferable to use a smaller $\Rr$ due to inaccurate estimate of to $\hbopt$. This explains why, in practice, lower dimensional representations may be preferable (see Fig. \ref{fig2}(d) for details).


%\mf{add a few lines on Notation?}

%\mf{mention the tilde O and lesssim notations. We can otherwise remove this parag, same notation described on page 1. unless we have other key notation from the rest of paper.}
\fi

\section{Related work}

\an{Think we need to add some more lines here about what our contributions are over-and-above these works in each category. Could maybe reduce the descriptions of original works and add broader summaries if we need to save space.}

\label{sec:related_work}
\noindent\textbf{Theory for representation learning} 
The recent papers \citep{kong2020meta,kong2020robust,tripuraneni2020provable, du2020few} propose the theoretical bounds of representation learning when the tasks lie in an exactly low dimensional (we call the dimension $\rt$) subspace, where the first three discuss method of moment estimators and the last two discuss matrix factorized formulations. \cite{tripuraneni2020provable} %proposes 
shows that 
%when features are $d$ dimensional and the task covariance matrix is exactly rank $\rt$ where $\rt\ll d$, 
the number of samples that enable meaningful representation learning is $\order{d\rt^2}$. \cite{kong2020meta,kong2020robust,tripuraneni2020provable} all assume that the features follow a standard normal distribution. We define a canonical covariance which handles arbitrary feature and task covariances. We also show that our estimator succeeds with $\order{d\rt}$ samples when $\nspt\sim\rt$.
%. We study the more general setting of arbitrary feature and task variances, and we show better sample complexity is achieved when the features and tasks are aligned. We also propose another estimator and it succeeds with $\order{d\rt}$ samples when $\nspt\sim\rt$.

\noindent\textbf{Subspace-based meta learning}
After representation learning is executed, we will use it to learn a new task generated from the same task distribution. \cite{kong2020meta,kong2020robust,tripuraneni2020provable, du2020few} assume that the task covariance is exactly low-rank, so they learn the new task in a subspace. 
%\mf{does this mean they assume $\Sigma_\beta$ is exactly low-rank? this will be more clear than saying 'tasks are low-dimensional'} 
%so they search for $\hbLa$ 
%\mf{what's the 'learning space'? say precisely what is projected} 
%in the low dimensional subspace and are able to learn with $\order{\rf}$ samples. We ask whether it is possible to search in the whole $d$ dimensional space with $\order{\rf}$ samples (in which case we have to train in an overparameterized regime). 
We investigate a representation with arbitrary dimension, specifically we are interested in overparameterized case -- does it yield a smaller error than low dimensional representation? This is meaningful especially when the feature/task covariances are approximately but not exactly low rank. \cite{yang2020provable,yang2021impact} study the sample efficiency of a low dimensional representation for learning linear bandits. \cite{lucas2020theoretical} analyzes the error of whole meta-learning procedure, called generalization error, and gives information theoretic lower and upper bounds. \cite{bouniot2020towards} studies more general tasks and metrics for subspace based meta-learning, such as classification problems, and analyzes the error with the impact of task diversity and proposes algorithms called metric-based and gradient based methods. Other slightly different settings involve learning low rank matrices \citep{chen2020learning} and functionals from a family of functions with covering number depicting its complexity \citep{garg2020functional}.

\ys{Adhyyan: Are you sure this is the proper sequence of related works? I feel the following paragraph is mixed lin regression and the last paragraph is subspace based meta learning.}
\an{Yes what you are saying makes sense. Does the new categorization work? From the description, mixed linear regression and subspace-based metalearning is seeming similar. Would it be possible to add a line or two to point the differences?}

\noindent\textbf{Mixed Linear Regression} A commonly studied %\mf{or `commonly studied';`reasonable'}   
setup is when tasks are generated from a Gaussian distribution $\Nn(0,\B)$, and %the majority of 
 $\B$ is exactly low rank or contains a %big 
large portion of small eigenvalues. 
This is studied as mixed linear regression \citep{zhong2016mixed, li2018learning, chen2020learning}, which consists of multiple linear regression problems. The knowledge of the distribution of the tasks, or the subspace where the tasks lie in,
% reduces the complexity of the search space and
enables robust and sample efficient learning for new tasks. \cite{lounici2011oracle,cavallanti2010linear,maurer2016benefit} propose sample complexity bounds of representation learning for mixed linear regression. There are study of mixed linear regression combined with other structures such as binary task vectors  \cite{balcan2015efficient} and sparse task vectors \citep{argyriou2008convex}. 

\noindent\textbf{Overparameterized ML and double-descent}
\cite{bartlett2020benign} analyzes the generalization guarantee of overparameterized linear regression, \cite{chang2020provable} extends it to non-linear models. \cite{nakkiran2020optimal,wu2020optimal} analyze ridge regression with weighted regularizer. The search space is the $d$ dimensional space, where $d$ is larger than the number of samples. By contrast, subspace based method which learns in a low dimensional subspace. The generalization guarantee is achieved by optimal ridge regression. %As a comparison, The subspace based method learns a low dimensional representation of the tasks, or the span/principal subspace of $\B$, where the dimension is smaller than the number of few-shot samples.
%In our work, 
%Compare with them,
%In comparison, 
We propose learning an (overparameterized) optimally-shaped representation 
%nd we study the two learning phases 
that we then use in the few-shot learning phase, providing an end-to-end performance study of meta-learning.
%and analyze its performance. 
%We further justify how this shaping is affected by representation learning, and analyze the end to end performance of meta-learning. 
%\mf{better but still not clear, maybe want to say that effectively we present an end-to-end study...}
%In the end we analyze the end to end 

\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|} 
 \hline
 & our work & subspace-based & overparameterization\\
 \hline\hline
 estimating data distribution & \checkmark & \checkmark & \xmark\\
 \hline
 arbitrary feature distribution & \checkmark & \xmark & \checkmark \\
 %\hline
 %subspace representation & \checkmark & \checkmark & \checkmark \\
 \hline
 overparametrized representation & \checkmark & \xmark & \checkmark \\
 \hline
 overparameterized rep learning & \checkmark & \xmark & \xmark \\
 \hline
 end to end error of meta-learning & \checkmark & \xmark & \xmark \\
 \hline
\end{tabular}
\vspace{.2em}
\caption{Related works}\label{table:works}
\end{table*}

\ys{
We compare our contributions with others in Table \ref{table:works}. Specifically:
\begin{enumerate}[leftmargin = *]
    \item We use representation learning to estimate data distribution. 
    \item Our method allows arbitrary feature/task covariance, as compared to \cite{tripuraneni2020provable,kong2020meta,kong2020robust} that assume $\bSi=\Ib$. When $\Bbar$ is spiked, the sample complexity can be lower than degree of freedom $\order{dr}$.
    \item We use $\hbLa\in\R^{R\times d}$ for representation. $R$ is arbitrary as compared to subspace-based method that learns a low dimensional representation.
    \item We propose the end to end bound of meta learning containing both representation and few-shot learning phases.
\end{enumerate}
}



==> sections/bc/setup_05_23.tex <==
\vspace{-.5em}
\section{Problem Setup}\label{sec:setup}

\textbf{Notation:} We describe each representation learning task using vector $\bt_i\in\R^d$, data samples are $(\xij,\yij)\in\R^d\times \R$, and noise $\eps_{ij}\in\R$. The distribution of $\bt_i$ and $\xij$ are $\Nn(0,\B)$ and $\Nn(0,\bSi)$. The rank of $\B$ and $\bSi$ are $\rt$ and $\rf$. The few-shot learning (downstream) task is $\bt$ and samples are $(\x_i, y_i)$. There are $\ntask$ tasks with $\nspt$ samples per task in the representation learning phase, and a few-shot learning task with $\nfs$ samples. Denote $\ntot = \ntask\nspt$. 
Let the representation matrix be $\hbLa\in\R^{R\times d}$.  We use $a\lesssim b$ or $\tilde\Order(b)$ that means there exists $K$ that depends logarithmically on all parameters such that $a\le Kb$.

The setup we consider consists of two phases: (i) representation learning, where prior tasks are used to learn a suitable representation, and (ii) few-shot learning, where a new task is learned with only a few samples. To aid in the theoretical analysis and understanding the generic behavior of the sample efficiency of general meta learning algorithms (see Fig. \ref{fig:fs_double_descent}), we study linear regression tasks, and focus on a setup where the tasks and the features per task are generated randomly.
%\mf{have to say something like ``to aid in the theoretical analysis and understanding the generic behavior of so-and-so learning schemes, we study linear regression tasks, and focus on a setup where the tasks and the features per task are generated randomly."}
%\mf{we decided this will be clarified at the start of the Problem Setup section.}

We assume that 
%representation learning and few shot learning
the two phases share the same distributions for features and tasks. 
\iffalse
If the task covariance matrix
%of the task 
is approximately low rank, 
%we hope to 
learning this structure in the representation learning phase can enable few-shot learning
%to work 
with fewer samples. 
%In the representation learning phase, 
%we learn the low dimensional space spanned by parameters. In the few-shot learning phase, we use the subspace to learn the model of a new task ideally with few samples.
\fi
In the first phase, there are multiple tasks, each with a batch of available data. The underlying task vectors are 
%to infer from, 
generated from the same distribution. 
%One accesses batches of data, each of whom is 
%collected from a task. %, however we may not know which task it comes from \mf{do we assume this?}. 
We make this setup more precise using the following definitions.


\begin{definition} \label{def:task}
\textbf{Representation learning: tasks.} 
Suppose the tasks are i.i.d. drawn from the distribution $\Nn(0, \B)$ where $\B\in\mathbf{S}^{d}_{+}$. %\mf{the common notation for symmetric matrices is $\mathbf{S}^d$}. 
We denote the $i$th task by $\bt_i\in\R^d$ and the number of tasks by $\ntask$.
%and there are in total $\ntask$ tasks. \vspace{-.3em}
\end{definition}

After we randomly draw tasks from the distribution, we generate data as defined below.


\begin{definition} \label{def:data}
\textbf{Representation learning: data per task.}
Fixing $\bt_i$, we generate features $\xij\in\R^d$, %\mf{remove the comma in the index and everywhere, as is in the intro} 
labels $\yij\in\R$ for $i=1,...,\nspt$, which follows $\yij = \xij^\top \bt_i + \eps_{ij}$. $\xij$ across all tasks are generated from $\Nn(0, \bSi)$.
%, and we assume $\bSi$ is approximately rank $\rf$ if needed
Without loss of generality, we assume $\bSi$ is diagonal (the task covariance $\B$ can be any positive semidefinite matrix). 
%$\eps_{ij}$, across all tasks, are generated 
$\eps_{ij}$ denotes the additive noise with distribution $\Nn(0, \sigma_\eps^2)$. For simplicity %in terms of scaling, 
we assume $\bSi$ and $\B$ are scaled so that $\|\bSi\|,\|\B\|\ge 1$. %\mf{is this the right scaling we need? looks strange} \ys{Yes for normalization we need a lower bound on their power, otherwise I need quite complicated normalization everywhere in thms}
\end{definition}

In Section \ref{sec:meta train} we %primarily 
study different estimators for %estimating 
the task covariance (or its low-rank approximation). 
%or its top eigenvectors. 
We assume 
$\B$ is rank $\rt$ and $\bSi$ is rank $\rf$. In general $\rt,\rf$ can be as large as $d$, 
but we will see the benefit when $\B,\bSi$ are approximately low rank. 
%We will use the estimation of $\B$ to form the optimal shaped representation.\mf{this should come before the `shaped' definition.}

%states different estimators and their error. Specifically, we estimate the task covariance and we can find the subspace spanned by task vectors. The result hold for all diagonal positive semidefinite (PSD) $\bSi$ and (not necessarily diagonal) PSD $\B$ matrices. As we mentioned at the beginning, we hope that $\B$ is (approximately) low rank, which means there is a low dimensional representation of tasks. We assume $\B$ is approximately rank $\rt$ and $\bSi$ is approximately rank $\rf$ if needed in our theorem.
%, which, when taking inner product of features, also indicates that there is a low dimensional feature representation. 
%, or use the subspace spanned by the top $\rt$ eigenvectors (where we hope $\lambda_r(\B) \gg \lambda_{\rt+1}(B)$) in few-shot learning phase. 
%If meanwhile $\bSi$ is approximately rank $\rf$, and the span of top $\rf$ eigenvectors of $\bSi$ covers the span of top $\rt$ eigenvectors of $\B$ (hence $\rf\ge \rt$), then the representation learning algorithm is further more sample efficient. 
Next we define the few-shot learning phase. 

\begin{definition} \label{def:few shot}
\textbf{Few shot learning.} In the few shot learning phase, suppose the task vector $\bt$ is generated from $\Nn(0, \B)$, the features $\x_i$, $i=1,...,\nfs$ are independently generated from $\Nn(0, \bSi)$, and $y_i = \x_i^\top\bt + \eps_i$ where noise $\eps_i$ 
are independently generated from 
$\Nn(0, \sigma_\eps^2)$.
\end{definition}

%In the few-shot learning phase, 
We investigate the training error and the sample efficiency for the few-shot learning phase with respect to the representation of data. 
%When we apply the training on the raw features without preprocessing, the algorithm requires $\Order(d)$ samples to learn a new task. 
In \cite{kong2020meta,kong2020robust,tripuraneni2020provable, du2020few}, the task covariance is assumed to be rank $\rt$ (i.e., representation of the features is $\rt$ dimensional). We propose a weighted representation of features as below, which is in general $R$ dimensional and the new task can be learned with $\Order(\rt)$ samples even if $R\approx d$.
%which is learned in representation learning. We propose a weighted representation of features, which keeps the features as $d$ dimensional, and the new task is learned with $\Order(\rt)$ samples as long as task covariance $\B$ is exactly or approximately $\rt$ rank. We will propose the optimal shaping and compare with the low dimensional representation. %Then we will propose a shaped representation of features.


\begin{definition}\label{def:weight}
\textbf{Shaped representation.} We define the weighted representation of features $\x$ with a shaping matrix $\hbLa_R\in\R^{R\times d}$ as $\hbLa_R\x$. 
\end{definition}

In the next section, we will learn the downstream task vector 
%\mf{what does retrieve mean here? do you mean "we will handle the downstream task..."}  \mf{i.e., the few-shot learning task described above} 
by finding the least norm solution with the shaped representation. The optimal shaping depends on the covariance of task and feature. Since we do not know their covariance, we use the covariance estimators in representation learning phase.


\begin{figure}[htbp!]
\centering
\includegraphics[width =0.5\linewidth]{figs/repl8.png}
\caption{Steps of meta-learning. Representation learning: Generate $\xij\in\Nn(0,\bSi)$ and $\bt_i\in\Nn(0,\B)$ and estimate $\yij = \xij^\top\bt_i$. $i\in[\ntask], j\in[\nspt]$. Use $\x$ and $y$ to learn $\hB$. Few-shot learning: Generate $\bt\in\Nn(0,\B)$ and $\x_i\in\Nn(0,\bSi)$, and estimate $y_i = \x_i^\top\bt$. $i\in[\nfs]$. Use $\x,y,\hB$ to estimate $\bt$.} 
\label{fig:meta learning}
\end{figure} 

In the upcoming sections, we will present the analyses of Algorithm \ref{algo:1} in two aspects: In Section \ref{sec:meta train}, we discuss the method of moments (MoM), which learns the task distribution from the dataset collected from multiple tasks. In Section \ref{sec:few shot}, we propose the optimal overparameterized representation of features, and show how to use the representation for few-shot learning. Finally we integrate the two parts and give an analysis of the overall meta-learning algorithm.



==> sections/checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{In supplementary file}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> sections/discussion_not_in_paper.tex <==
================== DELETE BELOW ==================
\subsection{One step GD}


\paragraph{What does this mean for gradient descent?} If we just look at the GD analysis in \cite{tripuraneni2020provable}, we can replace the Frobenius norm by $\tr(UV^\top \bSi VU^\top)$ in their bound, but the sample complexity cannot be smaller (like $(d+t)r\rightarrow(r+t)r$) to claim that all global minimums are good. Because there's no regularization in the objective (note that $\frac{1}{2}\|U^\top U - V^\top V\|$ is not a regularizer. If $ex^\top$ has a nullspace, you can always make both $U,V$ big in the null space but the value is $0$), and the analysis is based on overdetermined LS. So you can imagine that if the sample size gets slightly smaller, we are approaching the spike in the double descent curve, and when it gets through to overparameterized regime, we have to take the least norm solution and the landscape looks different.

So we need to add two things: early stopping or regularization. Now we consider the simple problem
\begin{align*}
    \min_{W\in\R^{t\times d}}\ \sum_{i=1}^n \|e_{t(i)}^\top W\x_i - y_i\|^2 
\end{align*}
We start from $W = 0$ and follow the gradient. Let $\tilde \B\in\R^{t\times d}$ be the matrix whose rows are the task vectors $\bt_j$, and let $\tilde \B_j$ be the matrix whose $j$th row is $\bt_j$ and the other rows are $0$. The gradient is 
\begin{align*}
    -\nabla f(W) &= \sum_{i=1}^n y_ie_{t(i)}\x_i^\top\\
    &= \sum_{i=1}^n e_{t(i)}\bt_{t(i)}^\top\x_i\x_i^\top + \eps_ie_{t(i)}\x_i^\top\\
    &= \sum_{i=1}^n \tilde \B_{t(i)} \bSi + \eps_ie_{t(i)}\x_i^\top.
\end{align*}
So 
\begin{align}
    \frac{1}{n}\mtx{E}(-\nabla f(W)) = \frac{1}{t} \tilde \B \bSi. \label{eq:gd_mean}
\end{align}
%So that we need $O(td)$ samples to estimate $W$, and if $\bSi$ is rank $r$, we need $O(tr)$ samples.
Now the variance analysis is easier. 
\begin{enumerate}
    \item Estimating the rows of $\tilde\B$. Fixing each $\bt_j$, we are just summing over $(\sum_i\ones(t(i) = j)\x_i\x_i^\top) \bt_j$. We know from Lemma \ref{lem:xxt} the concentration of $\sum_i\x_i\x_i^\top$ so we know how many samples we need to estimate each $\bt_j$.
    \item Estimating $\tilde\B\bSi$. We use $\frac{1}{n}\mtx{E}(-\nabla f(W))$ in \eqref{eq:gd_mean}. 
    The mean is $\frac{1}{t} \tilde\B\bSi$, the error decreases as
    \begin{align*}
        O(\sqrt{\frac{\tr(\bSi) \tr(\sbSi\B\sbSi) + 2\tr(\bSi\B\bSi)+ \sigma_\eps^2 \tr(\bSi)}{n}}).
    \end{align*}
    The proof is presented in latter sections.
\end{enumerate}
\paragraph{Matrix factorization.} Now we study the matrix factorization form 
    \begin{align*}
        \min_{\Ub\in\R^{t\times r}, \Vb\in\R^{d\times r}}\ \sum_{i=1}^n \|\eb_{t(i)}^\top \Ub\Vb^\top\x_i - y_i\|^2 := f(\Ub, \Vb)
    \end{align*}
    Denote $\A_i = \eb_{t(i)}\x_i^\top$, $\delta_i = y_i- \eb_{t(i)}^\top \Ub\Vb^\top\x_i$. We consider the gradient flow where 
    \begin{align}
        d\Ub / dt &= -\nabla_\Ub f(\Ub, \Vb)/dt = \sum_{i=1}^n \delta_i \A_i\Vb,\\
        \ d\Vb / dt &= -\nabla_\Vb f(\Ub, \Vb)/dt = \sum_{i=1}^n \delta_i \A_i^\top\Ub.
    \end{align}
    Note that
    \begin{align}
        d\Ub^\top\Ub / dt =  d\Vb^\top\Vb / dt \label{eq:inbal}
    \end{align}
    and
    \begin{align}
        df/dt &= -2\sum_{i=1}^n \delta_i(\langle\A_i, \sum_{i=1}^j(\delta_j \A_j \Vb\Vb^\top + \delta_j\Ub\Ub^\top \A_j) \rangle)\\
        &= -2( \langle\sum_{i=1}^n\delta_i\A_i, \sum_{i=1}^n\delta_i\A_i\Vb\Vb^\top\rangle + \langle\sum_{i=1}^n\delta_i\A_i,\Ub\Ub^\top \sum_{i=1}^n\delta_i\A_i\rangle)
    \end{align}
    Suppose the variables are initialized at $\Ub(0), \Vb(0)$ and follow the gradient flow, let the variables at time $\tau$ be $\Ub(\tau), \Vb(\tau)$. Then we know that $\sigma_i(\Ub(\tau)) - \sigma_i(\Vb(\tau)) = \sigma_i(\Ub(0)) - \sigma_i(\Vb(0))$ due to \eqref{eq:inbal}.
    
    Denote 
    \begin{align*}
        S(\Ub, \Vb) = \sum_{i=1}^n\delta_i\A_i
    \end{align*}
    then 
    \begin{align*}
        df/dt =-2( \langle S(\Ub, \Vb), S(\Ub, \Vb) \Vb\Vb^\top\rangle +  \langle S(\Ub, \Vb), \Ub\Ub^\top S(\Ub, \Vb)\rangle)
    \end{align*}
     and 
    \begin{align}
        d\Ub\Vb^\top / dt = 2( S(\Ub, \Vb) \Vb\Vb^\top + \Ub\Ub^\top S(\Ub, \Vb))
    \end{align}
    \iffalse
    What if we think about 
    \begin{align}
        d\Ub / dt &= (\Ib - \Pc_\Ub)\SUV\Vb,\\
        d\Vb / dt &= (\Ib - \Pc_\Vb)\SUV^\top\Ub
    \end{align}
    where $\Pc$ denotes the projection onto the column space. Then 
    \begin{align}
        d\Ub^\top\Ub / dt &=  d\Vb^\top\Vb / dt = 0\\
        df/dt &= -2( \langle\sum_{i=1}^n\delta_i\A_i, (\Ib - \Pc_\Ub)\sum_{i=1}^n\delta_i\A_i\Vb\Vb^\top\rangle + \langle\sum_{i=1}^n\delta_i\A_i,\Ub\Ub^\top \sum_{i=1}^n\delta_i\A_i (\Ib - \Pc_\Vb)\rangle)
    \end{align}
    \fi

    
    



%We use the approach in Section \ref{s:bernstein_short}. 
In brief, we only need to study the tail bound and variance of $ye\x^\top$. 


\iffalse
\begin{align}
    ye\x^\top &= (\x^\top\bt_{t(i)} + \eps_i) e\x^\top\\
    &= e\bt_{t(i)}^\top \x \x^\top + \eps_i e\x^\top
\end{align}
%whose norm is bounded by $\|\bt_{t(i)}\| \|\x \x^\top\|$. 
%We know the tail bound of $\|\x \x^\top\|$ from Section \ref{s:cov}
%, we just replace $K$ by $K = $. 
\begin{align}
    \mtx{P}(|\bt^\top \x| \ge t ) &\le \exp(-ct/ \|\sqrt{\B}\x\|)\\
    \mtx{P}(\|\sqrt{\B}\x\| - \tr(\sbSi\B\sbSi) \ge t) &\le \exp(c\min\{\frac{t^2}{\tr((\sbSi\B\sbSi)^2)}, \frac{t}{\|\sbSi\B\sbSi\|}\})\\
    \mtx{P}(\|\x\|^2 - \tr(\bSi) \ge t) &\le \exp(-c\min\{\frac{t^2}{\tr^2(\bSi)}, \frac{t}{\|\bSi\|}\})\\
    \mtx{P}(|\eps| \ge t) &\le \exp(-ct^2 / \sigma_\eps^2)
\end{align}
\fi
Now we bound $\|y\x\|$. With probability $1-\delta$, $\|x\|$ is bounded by \eqref{eq:norm_x_bd}, and $|y| = |\bt^\top\x| \le O(\|\sbSi\bt\|(1 + \sqrt{\log(1/\delta)}))$. Then with probability $1-\delta$
\begin{align*}
   \|y\x\| \le  (1 + \log(1/\delta))\tr(\bSi)\|\sbSi\bt\|.
\end{align*}
With probability $1-\delta$, we have 
\begin{align*}
    \|\sbSi\bt\| \le (1 + \sqrt{\log(1/\delta)})\sqrt{\tr(\sbSi\B\sbSi)}
\end{align*}
So with probability $1-\delta$, we have 
\begin{align}
    \|y\x\| \le  (1 + \log(1/\delta)^{3/2})\tr(\bSi) \sqrt{\tr(\sbSi\B\sbSi)}
\end{align}

    \begin{align}
        \mtx{E} \|y^2e\x^\top\x e^\top \| &= \mtx{E} (\x^\top\bt_{t(i)} + \eps_i)^2 \x^\top \x\\
        &= \frac{1}{t} \mtx{E} (\x^\top \tilde\B^\top\tilde\B \x\x^\top\x) + \sigma_\eps^2 \tr(\bSi) \label{eq:onestepgd_exp}
    \end{align}
    To compare it with other two parts, we switch to the case where $\bt$ is generated from $\mathcal{N}(0, \B)$ but we can replace $\frac{1}{t}\tilde\B^\top\tilde\B = \B$. 
    
We continue from \eqref{eq:onestepgd_exp}. Note that $\frac{1}{t}\mtx{E}(\tilde\B^\top\tilde\B) = \B$, let $\z\sim \mathcal{N}(0, I_d)$, so we have 
    \begin{align*}
        \mtx{E} \|y^2e\x^\top\x e^\top \| &= \mtx{E} (\x^\top \B \x\x^\top\x) + \sigma_\eps^2 \tr(\bSi) \\
        &= \mtx{E} (\z^\top \sbSi\B\sbSi \z\z^\top\bSi\z) + \sigma_\eps^2 \tr(\bSi).
    \end{align*}
    WLOG, we assume that $\bSi$ is diagonal (otherwise we can rotate by the eigenvectors of $\bSi$). Then 
    \begin{align*}
       \mtx{E} (\z^\top \sbSi\B\sbSi \z\z^\top\bSi\z)
        &= \sum_{i=1}^d \sigma_i \z^\top \sbSi\B\sbSi \z\z_i^2 \\
        &= \sum_{i=1}^d \sigma_i (\sum_{j=1}^d\sigma_j\B_{jj} + 2\sigma_i\B_{ii}) .\\
        &= \tr(\bSi) \tr(\sbSi\B\sbSi) + 2\tr(\bSi\B\bSi)
    \end{align*}
    The mean is $\frac{1}{t} \tilde\B\bSi$, the error decreases as
    \begin{align*}
        O(\sqrt{\frac{\tr(\bSi) \tr(\sbSi\B\sbSi) + 2\tr(\bSi\B\bSi) + + \sigma_\eps^2 \tr(\bSi)}{n}}).
    \end{align*}
    
    
    
\subsection{Robustness of Optimal Representation}
\begin{definition}[Optimal Representation] For a diagonal $\B$ the function $\opt(\cdot):\R^d\rightarrow\R^d$ solves the optimal representation problem \clr{\eqref{} subject to $\max_i(\opt_{i,i}(\B))/\min_i(\opt_{i,i}(\B))\leq C$ (in case we need nice conditioning)}. For a general $\B$ with eigendecomposition $\Ub\Eb\Ub^T$, set $\opt(\B)=\Ub\opt(\Eb)\Ub^T$.  %$\Bhat$ be the 
\end{definition}
\mf{let's change this as we discussed: make an assumption of same eigenspace like the Wu and Xu paper, then finding optimal ref reduces to diagonal}

Suppose $\bSi$ is identity. Let $\Bh$ be the estimate of the ground-truth task covariance $\B$. Let $\bLa$ and $\bLah$ be the optimal representations associated with $\B,\Bh$ respectively.

Given a few-shot task $\bt$ with associated training data $(\y,\X)$ define $\bth_\La$ and $\bth_\bLah$ obtained via \eqref{eq:min_norm}. \textbf{Important:} Note that we don't need to show closeness of $\La,\bLah$ (in terms of $\|\Bh-\B\|$). \clr{We just need to show that $\bLah$ achieves approximately same risk on the task distributions $\B,\Bh$ and $\La$ similarly achieves approximately same risk on $\B,\Bh$. By definition of optimality, this auto-implies $\bLah,\La$ achieves approximately the same risk and they are as good as each other!} 


As a result, we would like to argue that for any close pair $\B,\Bh$ the risk induced by (an arbitrary) representation $\La$ is close. \clr{To this aim, the first step is showing that $\bth_\La$ and $\bth_\bLah$ are close.}

Following \eqref{bSi test risk}, define the task averaged risk
\begin{align*}
\risk_{\B,\La}&=\E_{\bt\distas\Nn(0,\B)}[\risk_{\La}(\hat \bt_\La)]\\
&=\E_{\bt}[(\hat \bt-\bt)^\top \La^2(\hat \bt-\bt)].
\end{align*}
\clr{$\bullet$ TODO: Can we prove that?
\[
|\risk_{\Bh,\bLah}-\risk_{\B,\bLah}|\lesssim \tf{\B-\Bh}^2\quad\text{and similarly for $\La$}
\]}
\textbf{Possible considerations:} This is essentially Lipschitzness of the model with respect to the task distribution. Randomness of $\X$ might be a problem, i.e. what if it is bad-conditioned, pseudo-inverse might not be stable etc. Maybe we can use very small ridge regression in \eqref{eq:min_norm} to ensure $\bth_\La$ is well-behaved and small enough that the risk stays same.

\clr{\textbf{Final argument:} Combine this with the fact that $\risk_{\Bh,\La}\geq \risk_{\Bh,\bLah}$ (follows from the optimality of $\bLah$ for $\Bh$) implies the desired relation that $\bLah$ is good for distribution $\B$ i.e.
\[
\risk_{\B,\bLah}\leq \risk_{\Bh,\La}+C\cdot \tf{\B-\Bh}^2.
\]}



%The next step is showing the Lipschitzness of risk. 
%Observe that this is very related to Claim 1 as the risk difference can essentially be written in terms of $\La-\bLah$ and $\bth_\La-\bth_\bLah$.

%\textbf{Important:} Note that we don't need to show closeness of $\La,\bLah$ (in terms of $\|\Bh-\B\|$). We just need to show an upper bound on $\risk_{\B,\bLah}$.
%To show closeless of $\La,\bLah$ (in terms of $\|\Bh-\B\|$) one can use the fact that $\bLah$ is optimal for $\Bh$. This implies $\risk_{\Bh,\La}\geq \risk_{\Bh,\bLah}$.

\textbf{Alternative discussion:} If we can't prove the actual robustness, maybe prove/discuss it for representation with minimal bias which is simply $\La=\sqrt{\B}$ (from Xu/Wu paper).

Finally, we would like to use this robustness to prove an end-to-end learning bound with optimal representation (from representation learning to few-shot).

\clr{$\bullet$ TODO: State end-to-end bound. If necessary, *assume* the robustness of optimal rep OR use the rep with min bias\dots}

\ys{Did we estimate $\B$ in meta-training sec?}






\ys{Samet's approach.} We discuss the robustness with respect to the shaping matrix here. For any shaping matrix $\bL\in\R^{d\times d}$. Let $\bt\in\Nn(0,\B)$, $\y = \X\bt+\vct{\eps}$ where every row of $\X$ is independently from $\Nn(0, \bSi)$, we define $\bt_\bL = \bL(\X \bL)^\dag \y$, 
\begin{align*}
    \risk(\bL, \B) &= \Eb_{\x,\bt,\X,\y}(\bt - \bt_\bL)^\top\bSi(\bt - \bt_\bL)  + \sigma_\eps^2
\end{align*}
%\ys{Is this correct? How do you define the risk? The expression above, the expectation is taken over what, simply over $\x,\bt,\X,\y$?}

Denote
\begin{align*}
    \bLa = \arg\min_{\bL}\ \risk(\bL, \B),%\ \mbox{s.t.} \|\bL\|=1, \sigma_\min(\bL) > 1/\kappa.
\end{align*}
Thus $\bLa$ is the shaping that minimizes the risk. As we do not know $\B$, we use $\hat \bLa$ as the shaping matrix which is defined as  
\begin{align*}
    \hat \bLa = \arg\min_{\bL}\ \risk(\bL, \hB).
\end{align*}
From the optimality, we know that $\risk(\hbLa, \hB) \le \risk(\bLa, \B)$. 

Now we consider $\risk(\hbLa, \hB) - \risk(\hbLa, \B)$. 
\begin{align*}
    &\quad \risk(\hbLa, \B)\\
    &= \Eb(\bt - \hbLa(\X\hbLa)^\dag\y)^\top \bSi (\bt - \hbLa(\X\hbLa)^\dag\y)\\
    &= \Eb(\bt^\top \bSi \bt) - 2 \Eb(\bt^\top\bSi \hbLa(\X\hbLa)^\dag(\X\bt+\vct{\eps})) \\
    &\quad + \Eb\|\hbLa(\X\hbLa)^\dag(\X\bt+\vct{\eps})\|_{\bSi}^2\\
    &= \tr(\B\bSi) - 2 \Eb(\tr(\B\bSi \hbLa(\X\hbLa)^\dag\X)) \\
    &\quad +\Eb(\tr(\B[\hbLa(\X\hbLa)^\dag\X]^\top \bSi[\hbLa(\X\hbLa)^\dag\X] ) )\\
    &\quad + \sigma_\eps^2\tr([\hbLa(\X\hbLa)^\dag]^\top[\hbLa(\X\hbLa)^\dag])
\end{align*}
where each row of $\X$ is $\Nn(0,\bSi)$. Similarly 
\begin{align*}
    &\quad \risk(\hbLa, \hB)\\
    &= \tr(\hB\bSi) - 2 \Eb(\tr(\hB\bSi \hbLa(\X\hbLa)^\dag\X)) \\
    &\quad +\Eb(\tr(\hB[\hbLa(\X\hbLa)^\dag\X]^\top \bSi[\hbLa(\X\hbLa)^\dag\X] ) )\\
    &\quad + \sigma_\eps^2\tr([\hbLa(\X\hbLa)^\dag]^\top[\hbLa(\X\hbLa)^\dag])
\end{align*}
where each row of $\X$ is $\Nn(0,\bSi)$. We subtract them and get 
\begin{align*}
    &\quad |\risk(\hbLa, \hB) - \risk(\hbLa, \B)|\\
    &=\Big| \tr((\hB-\B)\bSi) - 2 \Eb(\tr((\hB-\B)\bSi \hbLa(\X\hbLa)^\dag\X))\\
    &\quad +\Eb(\tr((\hB-\B)[\hbLa(\X\hbLa)^\dag\X]^\top \bSi[\hbLa(\X\hbLa)^\dag\X] ) )\Big|\\
    &\le \|\hB - \B\|_F \cdot\left(\|\bSi\|_F + 2\|\Eb( \bSi \hbLa(\X\hbLa)^\dag\X) \|_F\right.\\
    &\quad\left. + \|\Eb([\hbLa(\X\hbLa)^\dag\X]^\top \bSi[\hbLa(\X\hbLa)^\dag\X])\|_F\right)
\end{align*}
\ys{$(\hbLa(\X\hbLa)^\dag\X)^2 = \hbLa(\X\hbLa)^\dag\X$, so that $eig(\hbLa(\X\hbLa)^\dag\X) = [{\bf 1}^m, {\bf 0}^{d-m}]$, not sure if this helps.}

We define the last line as $F(\hbLa, \bSi)\|\hB - \B\|_F$. Similarly we know that $ |\risk(\bLa, \hB) - \risk(\bLa, \B)| \le F(\bLa, \bSi)\|\hB - \B\|_F$.
So 
\begin{align*}
    &\quad \risk(\hbLa, \B) - \risk(\bLa, \B)\\
    &= \underbrace{\risk(\hbLa, \hB) - \risk(\bLa, \hB)}_{\le 0}\\
    &\quad + \risk(\hbLa, \B)-\risk(\hbLa, \hB)\\
    &\quad + \risk(\bLa, \hB)-\risk(\bLa, \B)\\
    &\le (F(\bLa, \bSi)+F(\hbLa, \bSi))\|\hB - \B\|_F.
\end{align*}

\ys{Multiplicative/additive error}

The risk in \ref{eq:risk_asy} is of the form 
$\risk(\B,\btheta) = \sum_{i=1}^d f_1(\btheta_i)\B_{ii} + f_2(\btheta)$. We need to make sure

1. If all $\max_i f_1(\btheta_i) = \bar f_1$, then if $\B$ is perturbed by $\delta$, $\risk$ changes at most $d\bar f_1$.

2. When $\B_{ii}$ is small, $f_1(\btheta_i)$ is not too big. Suppose 
\begin{align*}
    f_1(\btheta_i) &\le \bar f_1,\ \mathrm{if~}\B_{ii} \le \underbar{B}
\end{align*}
Then if $\B$ is perturbed by $\delta$,
\begin{align*}
    \risk(\B+\delta,\btheta) - \risk(\B,\btheta) \le \frac{\delta}{\underbar{B}}\risk(\B,\btheta) + d\bar f_1
\end{align*}




\ys{My thought from here}
Now we look at $\hat \bt = \bLa(\X\bLa)^\dag \y$. To show the robustness with respect to $\bLa$, we look at the matrix $\bLa(\X\bLa)^\dag$. Define a new matrix $\bL$ which is $\bLa$ after perturbation, and we will bound $ \bLa(\X\bLa)^\dag - \bL(\X\bL)^\dag$ by $\bLa - \bL$. $\X$ is a fat matrix and suppose it has full column rank, also suppose $\bLa, \bL$ be positive definite. Let $\X = \Ub[\bSi_\X,0][\Vb_1, \Vb_2]^\top$ be the SVD of $\X$. Let $\bLa = \Vb_1\bLa_1 + \Vb_2\bLa_2$, and $\bL = \Vb_1\bL_1 + \Vb_2\bL_2$.

First, $\X\bLa(\X\bLa)^\dag = \Ib = \X\bL(\X\bL)^\dag$ thus 
\begin{align*}
    \bLa(\X\bLa)^\dag - \bL(\X\bL)^\dag = \Vb_2\Vb_2^\top (\bLa(\X\bLa)^\dag - \bL(\X\bL)^\dag)
\end{align*}
Here $\Vb_2\Vb_2^\top$ is simply a projection matrix. Now we focus on $\Vb_2^\top (\bLa(\X\bLa)^\dag - \bL(\X\bL)^\dag)$.
\begin{align*}
    &\quad \Vb_2^\top (\bLa(\X\bLa)^\dag - \bL(\X\bL)^\dag)\\
    &= \bLa_2(\X\bLa)^\dag - \bL_2(\X\bL)^\dag\\
    &= \bLa_2(\Ub\bSi_\X\bLa_1)^\dag -  \bL_2(\Ub\bSi_\X\bL_1)^\dag
\end{align*}
Now we need to bound this quantity by $\bLa_1 - \bL_1$ and $\bLa_2 - \bL_2$, which are the perturbation of $\bLa$ projected onto the row space of $\X$ and its orthogonal complement.  

We continue with the expression and get
\begin{align*}
    &\quad \| \Vb_2^\top (\bLa(\X\bLa)^\dag - \bL(\X\bL)^\dag) \|\\
    &= \| \bLa_2(\Ub\bSi_\X\bLa_1)^\dag -  \bL_2(\Ub\bSi_\X\bL_1)^\dag \|\\
    &\le \|(\bLa_2 - \bL_2)(\Ub\bSi_\X\bLa_1)^\dag\|\\
    &\quad + \|\bL_2((\Ub\bSi_\X\bLa_1)^\dag - (\Ub\bSi_\X\bL_1)^\dag)\|\\
    &\le  \|(\Ub\bSi_\X\bLa_1)^\dag\| \|\bLa_2 - \bL_2\| \\
    &\quad + \|\bL_2\| \|(\Ub\bSi_\X\bLa_1)^\dag - (\Ub\bSi_\X\bL_1)^\dag\|\\
    &\le \|(\Ub\bSi_\X\bLa_1)^\dag\| \|\bLa_2 - \bL_2\| \\
    &\quad + \|\bLa_2\| \|\bSi_\X\| \| (\Ub\bSi_\X\bLa_1)^\dag \|^2 \|\bLa_1 - \bL_1 \| + o(\|\bLa - \bL\|)
\end{align*}
The last line uses the derivative of the pseudoinverse
\begin{align*}
    &\quad d((\Ub\bSi_\X\bLa_1)^\dag)\\
    &= (\Ub\bSi_\X\bLa_1)^\dag\Ub\bSi_\X (d\bLa_1)(\Ub\bSi_\X\bLa_1)^\dag\\
    &\quad + (I - (\Ub\bSi_\X\bLa_1)^\dag(\Ub\bSi_\X\bLa_1))\cdot\\
    &\qquad (d\bLa_1)^\top\bSi_\X\Ub^\top((\Ub\bSi_\X\bLa_1)^\dag)^\top(\Ub\bSi_\X\bLa_1)^\dag
\end{align*}


Similarly
\begin{align*}
    &\quad \| \Vb_2^\top (\bLa(\X\bLa)^\dag - \bL(\X\bL)^\dag) \|_F\\
     &\le \|(\Ub\bSi_\X\bLa_1)^\dag\| \|\bLa_2 - \bL_2\|_F \\
    &\quad + \|\bLa_2\|\|\bSi_\X\| \| (\Ub\bSi_\X\bLa_1)^\dag \|^2 \|\bLa_1 - \bL_1 \|_F
\end{align*}


================== DELETE ABOVE ==================

==> sections/experiments.tex <==


\section{Numerical Experiments}\label{sec:exp}
\vspace{-0.2em}
In this section, we will verify by experiments the three main contributions proposed before: (1) We apply the method of moment estimator for retrieving the covariance of the task or the top eigenspace.
We show that when feature space aligns with the task space, we only need $\order{\rf\rt^2}$ 
instead of $\order{d\rt^2}$ 
samples. (2) In Theorem \ref{thm:mom 1} part 2, we introduce task average estimator and argue that when each task contains $\Omega(\rt)$ samples, we can retrieve the subspace of tasks with $\order{\rf\rt}$ samples. 
(3) In Def. \ref{thm:opt rep theta}, we present the optimal representation matrix that minimizes the excess risk and in Theorem \ref{thm:e2e} we show the overall risk of meta learning algorithm. 

\paragraph*{Error of representation learning with respect to task feature alignment.} We depict this in Fig. \ref{fig2}(a). After applying method of moments estimators we do $\rt$-SVD truncation.
 We can see from Fig. \ref{fig2}(a) that, MoM's learn the subspaces accurately when $1 - \iota$ is large, (i.e., with feature-task alignment), whereas behave worse when $\bSi = \Ib$ Specifically, The MoM-F estimator works better only when $\iota$ is small, i.e., high task-feature alignment.


\paragraph*{Task average helps learning with fewer samples.} We show the sample efficiency of the task average estimator in Fig. \ref{fig2}(b). We fix the total number of samples $\ntot$, and vary the number of samples per task $\nspt$. In Theorem \ref{thm:mom 1} part 2, we argue that it estimates the task subspace with $\order{d\rt}$ samples when $\nspt \ge \rt$. We can see from the figure that, when $\nspt$ is small, this estimator degenerate to $\hat\Qb$ which asks for $\order{d\rt^2}$ samples, so the subspace estimation is bad. When $\ntask$ is small, the sampled task features cannot approximate the true task distribution, which also cause large error. We need $\nspt$ and $\ntask$ both reasonably large.

\paragraph*{Optimal representation.} In Fig. \ref{fig2}(c), we know $\B$ and do $R$-SVD truncation and apply optimal shaping for varying $R$. When the problem becomes overparameterized ($\nfs<R$), the estimation of downstream task depends on the shaping matrix. The risk corresponding to the optimal shaping matrix is smaller than using raw features for solving the downstream task.

\paragraph*{End to end behavior of meta-learning algorithm.} We run the whole meta-learning process. The normalized risk is plotted in Fig. \ref{fig2}(d). 
We use the optimal shaping matrix $\hbLa$, calculated as a function of $\hB$, for solving the downstream task. 
Both dimension reduction ($\nfs>R$) or optimal overparameterized problem ($\nfs<R$) end up with small risk, whereas it becomes hard to learn when $\nfs\approx R$. The risk of overparameterized case can be smaller than using low dimensional representation (typically applied in \cite{tripuraneni2020provable,kong2020meta,kong2020robust,du2020few}). 
As discussed in Remark \ref{rem:robust}, because we cannot learn $\B$ perfectly, the smallest risk with finite data happens when the chosen representation dimension $R<d$, unlike the case with known $\B$. 










==> sections/rep_learning_app.tex <==
%\vspace{-.5em}
\section{Representation Learning} 
\label{sec:meta train}

%\vspace{-.5em}
In the previous section, we derived the optimal choice of $\hbLa$ if we were provided with $\B$ and $\bSi$. In practice, the learner does not have access to these covariance matrices. Recall from Observation \ref{obs:canon} that the risk depends on the canonical covariance $\Bbar=\sbSi\B\sbSi$, so we only\footnote{We also need to estimate $\bSi$ for whitening. Estimating $\bSi$ is easy and has smaller error compared with $\Bbar$. The analysis is in first part of Appendix B.} need to estimate the $R$-dimensional principal subspace of $\Bbar$. Let us denote this subspace by $\mtx{S}$.
%and must instead estimate it from the data provided. In this section, we propose schemes for these estimations. First, we consider the following change of co-ordinates for our problem.

\iffalse
\begin{observation}[Equivalence to problem with whitened features]\label{obs:canon}
Given features $\x\sim\Nn(0,\bSi)$ and tasks $\bt\sim\Nn(0,\B)$, consider the change of co-ordinates $\tilde{\x}=\sbSiinv\x$ and $\tilde{\bt}=\sbSi \bt$ which ensures $\x^T\bt=\tilde{\x}^T\tilde{\bt}$ and leads to the canonical task covariance $\Bbar=\sbSi\B\sbSi$. Then
\[
\risk({\sbSi\hbLa},\B, \bSi) = \risk(\hbLa, \Bbar, \Ib)
\]
%\ys{put into last sec?}\mf{yes}
\end{observation}
\fi

\noindent\textbf{Sample complexity of subspace learning:} Recall that the representation has $Rd$ degrees of freedom. 
%Thus, intuitively, one needs at least $Rd$ examples. Closer to linear meta-learning, 
When $\Bbar$ is exactly rank $R$ and features are whitened, \cite{tripuraneni2020provable} provides a lower bound of $\Omega(Rd)$ examples and gives an algorithm achieving $\order{R^2d}$ samples. However, in practice, deep nets learn good representations despite overparameterization. In this section, we argue how inductive bias of the feature distribution can implicitly accelerate learning the canonical covariance. %Specifically, Figure \ref{} demonstrates that feature covariance is in fact positively correlated with the canonical task covariance for MNIST data. 
Inductive bias is found in practical instances. As an example, we trained $45={10\choose 2}$ SVM classifiers on MNIST each a binary classifier differentiating a pair of digits. The features are images and the task vectors are the support vectors. Here, we assessed correlation coefficient between two covariances via canonical-feature alignment defined as  {\color{red} $\frac{\text{trace}(\bSi^{1/2}\Bbar\bSi^{1/2})}{\|\bSi\|_F\|\Bbar\|_F}$} which generalizes the correlation coefficient for vectors. As reference, we compared it to canonical-identity alignment defined as  {\color{red} $\frac{\text{trace}(\Bbar)}{\sqrt{d}\|\Bbar\|_F}$} (replacing $\bSi$ with $\Ib$). The canonical-feature alignment score is $0.32$ whereas the canonical-identity alignment score is $0.15$. The similar quantity is verified on other datasets, shown in Fig. \ref{errM} (a) (b). This significant score difference exemplifies how $\bSi$ and $\Bbar$ can synergistically align with each other (inductive bias). This alignment helps our MoM estimator defined below, illustrated by Example \ref{example:spike} (spiked covariance).

%\ys{is this numerator correct? Or simply $\text{trace}(\Bbar)$?}

%This can be simply checked by plugging the transformed covariances into the expression for risk in the previous section in Equation~\ref{eq:bSi_test_risk}. Hence, the optimal representation $\hbLa^\ast$ for the original co-ordinates can be used to find the optimal for the new co-ordinates and vice versa. 

To develop a theory for representation learning, we propose the method-of-moment estimator towards this end. Our work differs from prior works such as \cite{kong2020meta,kong2020robust,tripuraneni2020provable} in two aspects:

%\SO{There are some repetitions throughout. We keep saying prior work is low-rank. It is good to emphasize this but no need to repeat 10 times. Instead let us focus on providing insights for our technical results.}
\begin{enumerate}[leftmargin=*]
    \item Prior works learn a \emph{low dimensional} subspace, whereas we estimate $\Bbar$ for overparameterized representation.
    %assume that the task covariance is exactly low rank, and use a \emph{low dimensional} subspace representation for the tasks. Our goal is to estimate $\Bbar$.
    \item Prior works assume that the feature covariance $\bSi = \Ib$. Let $r$ be task rank, the sample complexity is $dr^2$. %, as large as the degree of freedom (DoF) of $r$ dimensional subspace in $\R^d$, $\mathrm{Dof} = dr$. 
    Our learning guarantee holds for arbitrary covariance matrices $\bSi,\B$. The sample complexity depends on \emph{effective rank} and can be smaller than DoF. We use spiked covariance as an example below. 
    %With spiked covariances, we define effective ranks of covariance matrices and the sample complexity is $\order{\mathrm{rank}_{\mathrm{eff}}(\bSi)(\mathrm{rank}_{\mathrm{eff}}(\Bbar))^2}$. 
\end{enumerate}

%uses a \emph{low dimensional} subspace representation for the tasks. These works assume that the task covariance is exactly low rank, and aim to learn its span. Our learning guarantee holds for arbitrary covariance matrices $\bSi,\B$. To compare our result with earlier works, we also consider its implication for the case where $\Bbar$ has spiked eigenvalues as in Definition~\ref{def:spiked_covariance}.

%\an{The PCA subspace option is getting confusing because it has not been mentioned in problem setup or few shot section. Also this description should probably move to the setup section?}

%The representation $\hbLa$ can apply a simple subspace-based dimension reduction (\clr{PCA} option), as in \cite{kong2020meta,kong2020robust,tripuraneni2020provable}, or can be high-dimensional which allows for a \emph{softer} refinement of raw features by \emph{shaping} their covariance (Shaping option). We then use this feature representation in the few-shot learning phase on a new task to obtain a model $\hat\bt_{\hbLa}$ with small risk.

\iffalse
\setlength{\textfloatsep}{.2em}
\begin{algorithm}[htbp!]
\caption{Meta-learning. \an{Feel like this algorithm is making the same point as Figure 2 flow-chart in the setup section}}
\label{algo:1}
\begin{algorithmic}
 \REQUIRE{\emph{Representation learning data:} As in Phase 1.\\
 %\hspace{42pt}
 \emph{Few-shot learning data:} As in Phase 2.\\
 %Require 
 Value of $R$ if using PCA}
 %we reduce the features in $R$ dimensional dimension
\STATE{\hspace{-5pt}\textbf{Representation learning:} Calculate any moment estimator from Section \ref{sec:meta train}.}
\IF{\clr{PCA}}
\STATE{Let $\hbLa\in\R^{d\times R}$ be the projection to the span of top $R$ singular \new{vectors} of moment estimator.}
\ELSIF{Shaping}
\STATE{Calculate $\hbLa$ as defined in Def. \ref{thm:opt rep theta} and Thm. \ref{thm:opt rep theta}.} \an{But the definition uses $\B$ and not the moment estimator, no?}
\ENDIF
\STATE{\hspace{-5pt}\textbf{Few-shot learning:}}
\STATE{Calculate $\hat\bt_{\hbLa}$ from \eqref{def:minl2_interpolator}.}
\STATE{\textbf{Return:} $\hat\bt_{\hbLa}$.}
\end{algorithmic}
\end{algorithm}
\fi

%\so{please make clear our goal is estimating everything, but subspace is prticularly important\dots 
%and then make it clear, next secton goes beyond subspace and shows how everything is useful}


%Suppose the covariance of tasks $\B$ is approximately rank $\rt$.
%\clr{We want to estimate $\Sigma_\beta$ and other key variables that can be derived from it, in particular its principal eigenspace.}
%\clr{This principal eigenspace can be easier to estimate in the low-data regime\dots} 

%This section investigates the representation learning via method of moment estimators. 
%In general, %our result shows 
%recovery guarantees for arbitrary covariance matrices $\bSi$ and $\B$ if we have sufficient samples. 



%. Besides helping with the small risk in Phase 2., the spiked $\Bbar$ matrix is also shown to be learned with fewer samples in Phase 1.}
%We are particularly interested in the case when $\B$ and $\bSi$ are approximately low rank, so that we can estimate the moments with fewer samples. We define the effective rank of $\bSi$ as $\rf$ and the effective rank of $\B$ as $\rt$ later in the theorems. 
%As discussed above, we are interested in estimating $\sbSi\B\sbSi$ for the computation of optimal representation. %The theorems in this section apply to the case that $\x,\bt,\eps$ are subGaussian with the corresponding covariances.
%Estimating the moments is our primary goal, which can give full information about task covariance (if $\bSi = \Ib$, as we will show later). We can also obtain other key variables such as the principal eigenspace. 
%We are further interested in the case when the feature covariance $\bSi,\B$ are approximately low rank and their principal eigenspaces align. %In approximate low rank regime, our goal is to recover the span of top $\rt$ eigenvector of $\B$. 
%Based on this, we consider the method of moment estimators which will be defined later. 

%We summarize its performance in Table \ref{table:1}. %Suppose the rank of $\bSi$ is approximately $\rf$; we are interested in the $\rt<\rf\ll d$ case.



%\subsection{Method of moments} 

\begin{definition}[Method of Moment (MoM) Estimator]
\label{def:method_moment_estimator}
Define $\hat \bb_{i,1} = 2\nspt^{-1}\sum_{j=1}^{\nspt/2}\yij\xij$, $\hat \bb_{i,2} = 2\nspt^{-1}\sum_{j=\nspt/2+1}^{\nspt}\yij\xij$. Define 
\vspace{-1em}
\begin{align*}
    \hat \bM &= \nspt^{-1}\sum_{i=1}^{\ntask} (\bb_{i,1}\bb_{i,2}^\top + \bb_{i,2}\bb_{i,1}^\top),
\end{align*}
\vspace{-1em}

The expectation of $\hat \bM$ is $\bM = \bSi\B\bSi.$
\end{definition}


In our definition, we assume $\nspt\ge 2$, that there are at least $2$ samples per task. %, and we split the samples into two halves to compute  $\hat \bb_{i,1}$, $\hat \bb_{i,2}$. 
In \cite{tripuraneni2020provable}, $\nspt=1$ is allowed. We give the analysis of their estimator in appendix. The error is similar to $\hat\bM$.
\iffalse
We define $\hat \bb_i = \frac{1}{\nspt}\sum_{j=1}^{\nspt}\yij\xij$, for every $i=1,\ldots,\ntask$. Let $\hat \mfkb = [\hat \bb_1 \ldots \hat \bb_{\ntask}]$. Then the method of moment estimator is $\hat \BB = \frac{1}{\ntask} \hat \mfkb \hat \mfkb^\top.$ The expectation of this estimator $\hat \BB$ is 
 \begin{align*}
     \BB &:= \Eb(\hat \mfkb \hat \mfkb^\top) = \bSi\B\bSi  + \nspt^{-1}(\bSi\B\bSi + \tr(\B\bSi)\bSi + \sigma^2\bSi )
 \end{align*}
 And we discuss its error in the appendix.
 
 \an{I think this notation with so many different r's could definitely use some work. I think that we should replace $r_f$ with $s_f$ and $r_t$ with $s_t$. And then save the r's for the effective rank notation. But the different hats/bars/subscripts are getting very confusing here.} 
 \fi 
 
 In the following subsections, let $\ntot = \nspt \ntask$ refer to the total tasks in representation-learning phase. %let $\Snorm = \max\{\|\bSi\|, \|\B\|\}$, %$\TbtXsq = \tr(\B\bSisq)$,
 Let $\TX = \tr(\bSi)$, $\Tbt = \tr(\B)$, and $\TbtX = \tr(\Bbar)$.
 We have two results for this estimator.%, summarized in Table~\ref{table:1}:
 \begin{enumerate}[leftmargin=*]
     \item Generally, we can estimate $\bM $ with $\Order(\TX\TbtX^2)$ samples.
     \item With a definition of effective feature rank $\rf$, let $\nspt\ge \rt$, we can estimate $\bM$ with $\Order(\rf\rt)$ samples.
 \end{enumerate}
  \cite{tripuraneni2020provable} has sample complexity $\Order(dr^2)$ ($r$ is exact rank). If we replace $d,r$ by our effective ranks $\TX,\TbtX$, we map to our result $\Order(\TX\TbtX^2)$. So $\TX , \TbtX$ can be seen as effective ranks %of corresponding matrices 
  and our bounds are always smaller than $d,r$ of the setting in \cite{tripuraneni2020provable}. We will discuss later in Example \ref{example:spike}. Our second result says when $\nspt\ge \rt$, our sample complexity achieves the $\order{dr}$ lower bound in \cite{tripuraneni2020provable}.
%\an{Should this be $\TX$ and $\Tbt$ instead of $\rf$ and $\rt$ in the second point.}
\setlength{\textfloatsep}{.3em}
\begin{table}[t!]
\centering
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|c|c|} 
 \hline
  feature cov & \multicolumn{3}{|c|}{$\bSi = \Ib$, $\B=\diag{\Ib_{\rt},{\bf 0}}$} & \multicolumn{3}{|c|}{
  \makecell{$\bSi = \diag{\Ib_{\rf},\iotaF\Ib_{d-\rf}}$,\\ $\B=\diag{\Ib_{\rt},\iotaT\Ib_{d-\rt}}$}
  %{$\bSi = \diag{\Ib_{\rf}, 0}$}
  } \\
   \hline
 estimator & sample $\ntot$ & sample $\nspt$ & error & sample $\ntot$ & sample $\nspt$ & error\\
 \hline\hline
 MoM & $d\rt^2$ &$1$ & $(d\rt^2/\ntot)^{1/2}$ & 
 %$\rf\rt^2$ &$1$ & $(\rf\rt^2/\ntot)^{1/2}$ \\
 $\barrf \barrt^2$ & $1$ & $(\barrf \barrt^2/\ntot)^{1/2}$\\
 \hline
 MoM & $d\rt$ &  $\rt$ & $(\rt/\nspt)^{1/2}$ & $\barrf\barrt$ & $\barrt$ & $(\barrt/\nspt)^{1/2}$ \\
 %\hline
 %MoM-F & 
 %$d$ & $(d/\ntot)^{1/2}$ 
 %- & - & $\rf,1$ & $(\rf/\ntot)^{1/2}$ \\
 \hline
\end{tabular}
}
\vspace{.5em}
\caption{Sample complexity and error of MoM estimators. %Suppose $\B=\diag{\Ib_{\rt},{\bf 0}}$. $\iotaT, \iotaF\in(0,1)$, 
$\rf,\rt$ stand for feature, task approximate rank. $\barrf = \rf + \iotaF(d-\rf)$, $\barrt = \rt + \iotaT(d-\rt)$. % MoM-F is defined in appendix.
%\an{Should the $s$ be $r$ on the left side?}
Additionally, for the well-studied setting of identity feature and low-rank task covariance (left side), our bound in the second row is the first result to achieve optimal sample complexity of ${\cal{O}}(ds_{T})$ (cf.~\cite{tripuraneni2020provable, kong2020meta}).
}
\label{table:1}
\end{table}

\begin{theorem}\label{thm:mom 1}
Let data be generated as in Phase 1. Assume $\|\bSi\|, \|\B\|\ = 1$ for normalization\footnote{This is simply equivalent to scaling $\yij$, which does not affect the normalized error $\|\hat\bM - \bM\| / \|\bM\|$. In the appendix we define $\Snorm = \max\{\|\bSi\|, \|\B\|\}$ and prove the theorem for general $\Snorm$.}
\begin{enumerate}[leftmargin=*]
    \item Let $\nspt$ be a even number. 
Then there is a constant $c>10$, with probability $1 - \ntot^{-c}$,
\begin{align*}
   \| \hat \bM - \bM \| \lesssim (\TbtX + \sigma^2)\sqrt{\frac{\TX}{\ntot}} + \sqrt{\frac{\Tbt}{\ntask}}.
\end{align*}
\item 
Let $T \gtrsim \min \ \rf: \rf \ge d\lambda_{\rf+1}(\bSi)$. If $\nspt \gtrsim (\TbtX+\sigma^2)\Snorm$, then with probability $1 - \Order(\ntask^{-C_1} + (\ntask\TbtX)^{-C_2} + \exp(-C_3\ntask^2))$, where $C_i$ are positive constants, 
\begin{align*}
\| \hat \bM - \bM \| \lesssim \left((\TbtX+\sigma^2)/\nspt\right)^{1/2}. %\sqrt{\frac{\TbtX+\sigma^2}{\nspt}}
\end{align*}
\end{enumerate}
Suppose the top $R$ principal subspace of $\bM, \hat \bM$ are $\W, \hat \W$, and $\lambda_R(\bM) - \lambda_{R+1}(\bM) > \| \hat \bM - \bM \|$, then a direct use of \cite{davis1970rotation} says the angle between them satisfy \[\sin(\angle \W, \hat \W) \lesssim (\lambda_R(\bM) - \lambda_{R+1}(\bM) - \| \hat \bM - \bM \|)^{-1}\| \hat \bM - \bM \|.\]
\end{theorem}


\begin{figure}[t!]
\centering
%\vspace{-1em}
\subfigure{
\includegraphics[width =0.45\textwidth]{figs/align_err_YS2.eps}
}
\subfigure{
\includegraphics[width =0.45\textwidth]{figs/cor_datasets.eps}
}
\caption{(a) Error of MoM estimator. (b) Alignment of feature-task on image classification models.} \label{errM}
\end{figure} 

\noindent\emph{Estimating eigenspace of canonical covariance.} Note that if $\bSi$ and $\B$ are aligned, (e.g.~Example \ref{example:spike} below), then $\W=\mtx{S}$ is exactly the principal subspace of $\Bbar$. Thm. \ref{thm:mom 1} indeed gives estimation error for the principal subspace of $\Bbar$. Note that, such alignment is strictly weaker and more general requirement compared to related works which require whitened features \cite{tripuraneni2020provable, kong2020meta}.

%We have a direct generalization from \cite{kong2020meta,tripuraneni2020provable} to arbitrary covariance.
 %This result corresponds to the first line of Table \ref{table:1}. We defer the details the details and the proof to the appendix. 
 %To explain our theorem, 
 We use spiked $\Bbar$ for the example below. This characterization was inspired by recent interest in spiked covariance models \cite{wang2017spiked, mahdaviyeh2020risk} and %also its prevalence in 
 the double-descent literature.
%The sample complexity and error depends on DoF of $\bSi,\B$, related to the rank. 
%If the covariances have spiked spectral, we can define the \emph{effective} DoF which is reflected in the error in Thm. \ref{thm:mom 1}. %We will illustrate the theorem using bilevel $\bSi$ and $\B$ below.

%\an{We should give some intuition for the proof of the theorem here (Bernstein bound etc.). Further, we should make some commentary on the scalings. Like we were saying last meeting about the effective rank, correlation etc.}

%To illustrate the theorem, we consider the specific choice of bilevel $\Sigf$ and $\Sigt$. We find that the more spiked the spectrum is, the smaller the error in estimation is: the error increases with $\rf$ and $\rt$ and decreases with $\iotaF$ and $\iotaT$.

\iffalse
\new{
To illustrate the theorem, we consider a specific choice of $\bSi$ and $\B$. We have $\bSi$ approximately low-rank, with the first $r$ eigenvalues significantly larger than the others; the ratio of the large to small eigenvalues is controlled by the hyperparameter $\iota$. This characterization was inspired by recent interest in spiked-covariance models \cite{wang2017spiked, mahdaviyeh2020risk}. The task covariance, $\B$, is low rank and has only $\rt$ nonzero entries; this is inspired by the subspace-based meta-learning works described in Section~\ref{sec:related_work}.
}
\an{In this case, we find that .....}
\fi



\begin{example}[Spiked $\Bbar$, Aligned principal subspace]\label{example:spike}
%Suppose $0\le\iota\le 1$ $\bSi = \diag{\Ib_{\rf},\iotaF\Ib_{d-\rf}}$, and $\B = \diag{\Ib_{\rt}, \iotaT\Ib_{d-\rt}}$, $\sigma = 0$. 
Consider the specific case of when the spectra of $\bSi$ and $\Bbar$ follow the bilevel decay $\bSi = \diag{\Ib_{\rf},\iotaF\Ib_{d-\rf}}$, $\B=\diag{\Ib_{\rt},\iotaT\Ib_{d-\rt}}$. 
When $\rf>\rt$, the error in recovery of $\bM$ is bounded as \footnote{The second term can also be written as $\sqrt{\barrt\nspt/\ntot}$. Typically $\rt\gtrsim \nspt$ so the first term is larger.}
\[
     \|\hat \bM - \bM\|
     %\lesssim \sqrt{\frac{(\rt + \iotaT(\rf-\rt) + \iotaF\iotaT(d-\rf))^2\barrf}{\ntot}} + \sqrt{\frac{\barrt}{\ntask}} 
     \lesssim \sqrt{\frac{\barrt^2\barrf}{\ntot}} + \sqrt{\frac{\barrt}{\ntask}}.
\]
\end{example}



In Fig. \ref{errM} (a) we plot the error of estimating $\bM$ (whose principal subspace coincides with $\Bbar$). $\bSi=\diag{\Ib_{30},\iota \Ib_{70}}$, $\B=\diag{\Ib_{30},{\bf 0}_{70}}$. $\ntask = \ntot = 100$. We can see that the error increase with $\iota$.




\iffalse
\ys{
%We can see that, the top eigenvalue of $\bM$ is $1$, and when $\iotaF,\iotaT$ decrease, which means the matrix $\bM$ is more spiked, the spectral norm error of $\bM$ decreases.

\begin{example}[Spiked $\Bbar$, Misaligned principal subspace]
Now, consider the case $\bSi$ and $\B$ are missaligned. Let $\bSi = \diag{\iotaF\Ib_{\rf},\Ib_{d-\rf}}$, $\B=\diag{\Ib_{\rt},\iotaT\Ib_{d-\rt}}$, where $\rf+\rt<d$, and $0<\iotaF,\iotaT<1$. Then,

\begin{enumerate}[label=\textbf{\arabic*}), leftmargin=*, align=left]
    \item \begin{align*}
     \|\hat \bM - \bM\| &\lesssim (\iotaT\rf +\iotaF\rt + \iotaF\iotaT(d-\rt-\rf))\sqrt{\frac{\barrf}{\ntot}} + \sqrt{\frac{\barrt}{\ntask}}.
    \end{align*}
    \item Further, if $\iotaF^2< \iotaT$,
    \begin{align*} 
    |\hat \bM - \bM\|/\|\bM\| &\lesssim (\barrf + \frac{\iotaF}{\iotaT}\rt)\sqrt{\frac{\barrf}{\ntot}} + \sqrt{\frac{\barrt}{\ntask}}.
    \end{align*}
\end{enumerate}
\end{example}

Let us compare the two cases above. Recognize that the top eigenvalue of $\bM$ is upper bounded by $\max\{\iotaF^2,\iotaT\}$. If $\iotaF^2\ge \iotaT$, then $\|\hat \bM - \bM\|/\|\bM\|$ is $\iotaF^{-1}$ times the aligned case above. The first term for aligned case was $\barrt$. If $\barrf \ge \barrt$ (which can be true if $\rf>\rt$), then the normalized error for missaligned case is larger. Moreover, we notice that for computing the optimal representation matrix, the matrix we target to estimate is $\sbSi\B\sbSi$, and MoM estimates $\bSi\B\bSi$. When the missalignment is large enough, the two targets can have different principal subspaces.
}

\fi




\textbf{Implicit bias in representation learning:} Note that, in population limit, MoM estimator returns
\[
\M=\bSi\B \bSi=\sbSi\Bbar\sbSi.
\]
Here, canonical covariance is the attribute of interest and feature covariance $\sbSi$ terms implicitly modulates the estimation procedure. If our goal is estimating the principle canonical subspace, the degree of alignment between $\bSi$ and $\Bbar$ can make or break the estimation procedure.






\iffalse
\begin{corollary}
\label{cor:dr}(Standard normal feature, noiseless)
Let data be generated as in Phase 1. Suppose $\sigma = 0$, $\bSi = \Ib$, and suppose the rank of $\B$ is $\rt$.
Define $\hat \bt_j = \nspt^{-1}\sum_{j=1}^{\nspt}\yij\xij$,  $\mfkb = [\bt_1,...,\bt_{\ntask}]$, and $\hat \mfkb = [\hat \bt_1,...,\hat \bt_{\ntask}]$. Let $\nspt>c_1\Tbt\lambda^{-1}_{\rt}(\B)$, $\ntask>c_2\max\{d, \frac{\Snorm\Tbt}{\lambda_{\rt}^2(\B)}\}$,
%$\nspt>c_1\tr(\B)\lambda^{-1}_{\rt}(\B)$, $\ntask>c_2\max\{d, \frac{\|\B\|\tr(\B)}{\lambda_{\rt}^2(\B)}\}$, 
with probabilty $1 - (\ntask^{-c_3} + (\ntask \Tbt)^{-c_4} + \exp(-c_5\ntask^2))$, where $c_i$ are constants, $c_{3,4} > 10$, 
\begin{align*}
    \sigma_{\max}(\hat \mfkb - \mfkb) \lesssim \sqrt{\frac{\ntask \Tbt}{\nspt}}.
\end{align*}

Denote the span of top $\rt$ singular column vectors of $\hat \mfkb$ and $\B$ as $\hat \W, \W$, then
\begin{align*}
    \sin(\angle\hat \W, \W) \lesssim \sqrt{\frac{\Tbt}{\nspt\lambda_{\rt}(\B)}}.
\end{align*}

If $\B = \diag{\Ib_{\rt},0}$, then $\sin(\angle\hat \W, \W) \lesssim \sqrt{\rt/\nspt}$.
\end{corollary}

\begin{remark}
Theorem \ref{cor:dr} requires $\nspt>c_1\Tbt\lambda^{-1}_{\rt}(\B)$, so $\nspt$ is lower bounded by $\order{\rt}$ in Theorem \ref{cor:dr}. If $\nspt = 1$ and we estimate $\hat \mfkb$, then $\ntask\hat \Qb = \hat \mfkb\hat \mfkb^\top$. This means Theorem \ref{thm:mom} can be applied to this estimator when $\nspt = 1$.
\end{remark}
\ys{put in appendix}
\subsection{Estimating the covariance of features}
As we have defined in Def \ref{def:data}, features $\xij$ are generated from $\Nn(0,\bSi)$. We aim to estimate the covariance $\bSi$. Although there are different kinds of algorithms, such as maximum likelihood estimator \cite{anderson1970estimation}, to be consistent with the algorithms in the latter sections, we study the sample covariance matrix defined by \eqref{eq:bsi_est}.
\iffalse
%Note that the features across all tasks are generated from the same distribution, so we don't need to differentiate which task the data is generated from. From now on we %denote $\ntot = \nspt k$, and 
rewrite \eqref{eq:bsi_est} as 

\begin{align}\label{eq:bsi_est_2}
    \hbSi = \sum_{i=1}^{\ntot} \x_i\x_i^\top\vspace{-.6em}
\end{align}
where $\x_i\sim\Nn(0,\bSi)$. We have 
\fi
\begin{lemma}\label{lem:xxt}
Suppose $\xij$ are generated independently from $\Nn(0, \bSi)$. We estimate \eqref{eq:bsi_est}, then when $\ntot\gtrsim\TX$, with probability at least $1 - (\ntot\tr(\bSi))^{-10}$,
%$\ntot>\log^2(\tr(\bSi))\tr(\bSi)$, with probability $1 - \Order((\ntot\tr(\bSi))^{-C})$,

\begin{align*}
    \|\hbSi - \bSi\| \lesssim \sqrt{\frac{\Snorm\TX}{\ntot}}
\end{align*}
%\begin{align*}
%    \|\hbSi - \bSi\| \le \tilde \Order(\sqrt{\frac{\|\bSi\|\tr(\bSi)}{\ntot}})
%\end{align*}
Denote the span of top $\rf$ eigenvectors of $\bSi$ as $\W$ and the span of top $\rf$ eigenvectors of $\hbSi$ as $\hat \W$. Let $\delta_{\lambda} = \lambda_{\rf}(\bSi) - \lambda_{\rf+1}(\bSi)$. Then if $\ntot \gtrsim \frac{\Snorm\TX}{\delta_{\lambda}^2}$,
%\begin{align*}
%    \ntot \ge \tilde \Order(\frac{\|\bSi\|\tr(\bSi)}{(\lambda_{\rf}(\bSi) - \lambda_{\rf+1}(\bSi))^2})
%\end{align*}
we have 
\begin{align*}
    \sin(\angle\W,\hat\W) \lesssim \sqrt{\frac{\Snorm\TX}{\ntot\delta_{\lambda}^2}}
\end{align*}
%\begin{align*}
%    \sin(\angle\W,\hat\W) \sim \tilde \Order\left(\sqrt{\frac{\|\bSi\|\tr(\bSi)}{\ntot(\lambda_{\rf}(\bSi) - \lambda_{\rf+1}(\bSi))^2}}\right)
%\end{align*}
%\begin{align*}
%    &\|\hbSi - \bSi\| \le \tilde \Order\left( \log(\ntot\tr(\bSi))\right.\\
%    &\left.(\frac{\log(\ntot\tr(\bSi))\tr(\bSi)}{\ntot} + \sqrt{\frac{\|\bSi\|\tr(\bSi)}{\ntot}}) \right)
%\end{align*}
\end{lemma}
\iffalse
Now we will study the accuracy of this estimator in approximate low rank scenario. Suppose $\bSi$ is approximately rank $\rf$ and we are interested in the subspace of top $\rf$ eigenvectors. 
\begin{corollary}\label{cor:angle}
We use $\lambda_i$ to denote $i$th largest eigenvalue of $\bSi$. Suppose $\bSi$ is approximately rank $\rf$, and we do $\rf$ PCA to recover the subspace of top $\rf$ eigenvectors. Denote the subspace of top $\rf$ eigenvectors of $\bSi$ as $\W$ and the subspace of top $\rf$ eigenvectors of $\hbSi$ as $\hat \W$. Then if 
\begin{align*}
    \ntot \gtrsim \frac{\|\bSi\|\tr(\bSi)}{(\lambda_{\rf}(\bSi) - \lambda_{\rf+1}(\bSi))^2}
\end{align*}
we have 
\begin{align*}
    \sin(\angle\W,\hat\W) \lesssim \sqrt{\frac{\|\bSi\|\tr(\bSi)}{\ntot(\lambda_{\rf}(\bSi) - \lambda_{\rf+1}(\bSi))^2}}
\end{align*}
\end{corollary}
\fi 
\begin{example}
When $\bSi = \diag{\mtx{I}_{\rf}, 0}$, we have $\sin(\angle\W,\hat\W) \lesssim \sqrt{\frac{\rf}{\ntot}}$.
\end{example}

Lemma \ref{lem:xxt} gives the quality of the estimation of the covariance of features $\x$. %The error with respect to the number of samples is $\sqrt{\frac{\Snorm\TX}{\ntot}}$. 
When the condition number of the matrix $\bSi$ is close to $1$, we need $\ntot\gtrsim d$ to get an estimation with error $\Order(1)$. However, when the matrix $\bSi$ is close to rank $\rf$, the amount of samples to achieve the same error is smaller, and we can use $\ntot \gtrsim \rf$ samples to get $\Order(1)$ estimation error. 
\fi


